CSCPR: Cross-Source-Context Indoor RGB-D Place Recognition

We extend our previous work, PoCo, and present a new algorithm, Cross-Source-Context Place Recognition (CSCPR), for RGB-D indoor place recognition that integrates global retrieval and reranking into an end-to-end model and keeps the consistency of using Context-of-Clusters (CoCs) for feature processing. Unlike prior approaches that primarily focus on the RGB domain for place recognition reranking, CSCPR is designed to handle the RGB-D data. We apply the CoCs to handle cross-sourced and cross-scaled RGB-D point clouds and introduce two novel modules for reranking: the Self-Context Cluster (SCC) and the Cross Source Context Cluster (CSCC), which enhance feature representation and match query-database pairs based on local features, respectively. We also release two new datasets, ScanNetIPR and ARKitIPR. Our experiments demonstrate that CSCPR significantly outperforms state-of-the-art models on these datasets by at least 29.27% in Recall@1 on the ScanNet-PR dataset and 43.24% in the new datasets. Code and datasets will be released.

==> archive/v1.tex <==
\begin{abstract}
We present a new algorithm, Cross-Source-Context Place Recognition (CSCPR), for RGB-D indoor place recognition that integrates global retrieval and reranking into a single end-to-end model. Unlike prior approaches that primarily focus on the RGB domain, CSCPR is designed to handle the RGB-D data. We extend the Context-of-Clusters (CoCs) for handling noisy colorized point clouds and introduce two novel modules for reranking: the Self-Context Cluster (SCC) and Cross Source Context Cluster (CSCC), which enhance feature representation and match query-database pairs based on local features, respectively. 
We also present two new datasets, ScanNetIPR and ARKitIPR. Our experiments demonstrate that CSCPR significantly outperforms state-of-the-art models on these datasets by at least $36.5\%$ in Recall@1 at ScanNet-PR dataset and $44\%$ in new datasets. Code and datasets will be released.

\end{abstract}

% \keywords{RGB-D Indoor Place Recognition RGB-D datasets}


\section{Introduction}
\label{sec:intro}

Place recognition plays an important role in robotics~\cite{ijcai2021p603, lowry2015visual, liu2023survey, yurtsever2020survey}, \rev{where given query frames the goal is to identify matches from a database that share overlapping field of view with queries based on image similarities}~\cite{kornilova2023dominating, liu2023survey, yurtsever2020survey}. It is used in various applications, such as augmented reality~\cite{middelberg2014scalable}, navigation~\cite{mirowski2018learning, yurtsever2020survey}, SLAM~\cite{yurtsever2020survey, bresson2017simultaneous}, etc. However, the place recognition problem is very challenging~\cite{liu2023survey,yurtsever2020survey, lowry2015visual} due to: (1) different sensors, RGB, RGB-D, Lidar, etc., which require modality-specific feature processing; (2) Environmental challenges, such as illumination changes, dynamic objects, occlusion, and scale variation; (3) RGB-D indoor place recognition is not well studied~\cite{cgis, yurtsever2020survey, lowry2015visual}, where most of the current approaches only use global retrieval for place recognition~\cite{cgis, du2020dh3d}. Our approach focuses on the less explored domain of RGB-D indoor place recognition, and proposes an end-to-end architecture to handle both global retrieval and reranking.



\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{figs/front.jpg}
    \caption{\textbf{Real-world Experiment:} We propose a novel approach Cross-Source-Context Place Recognition (CSCPR) for RGB-D indoor place recognition. Given a query frame, global retrieval ranks the potentially matched frames, and our novel place-recognition reranking model reranks the candidates to achieve better recognition accuracy.}
    \label{fig:front}
    \vspace{-2em}
\end{figure}


\textit{RGB-D indoor place recognition is not well studied:} 
Visual place recognition has been explored for many years, especially in RGB domain~\cite{lowry2015visual, ijcai2021p603}. However, the potential of RGB-D data is overlooked, especially for indoor environments the depth information can be crucial for place recognition~\cite{cgis, du2020dh3d, lowry2015visual}. Traditional approaches rely on global retrieval, which extracts global descriptors from each frame and ranks the database frames by the similarities with the query frame~\cite{cgis, uy2018pointnetvlad, arandjelovic2016netvlad, yurtsever2020survey}. For RGB-D place recognition, we need to handle different modalities of perceptions (color and geometry), so a good feature extractor is critical in the global retrieval. In recent years, the CoCs~\cite{cocs} method has been proposed and demonstrated with comparable performance with attention mechanism~\cite{vaswani2017attention}, but less computational cost. In our approach, CSCPR, we take advantage of the concept of CoCs, which uses higher-level global information to enhance local features and propose a novel end-to-end architecture for place recognition jointly integrating both global and local features.

\textit{RGB-D place-recognition reranking is not well studied:} 
% Besides comparing the global descriptors, 
Reranking, as a complement to global retrieval, is to improve the accuracy by evaluating the matches of local features between the query and database frames~\cite{zhu2023r2former, hausler2021patch, vidanapathirana2023spectral}. Therefore, the reranking stage should be fast and accurate in matching local features. The RANSAC-based~\cite{ransac} methods are widely used for reranking by processing the geometric information of query-database frames~\cite{hausler2021patch, vidanapathirana2023spectral}. 
% tan2021instance
However, these methods only process hand-crafted geometric relations and ignores the color or other empirical features. Recently, learning-based approaches~\cite{zhu2023r2former, lee2022correlation} have been proposed that match empirical local features. However, those approaches are all for RGB-only place recognition. In this work, we generalize the learning-based reranking concept to RGB-D point cloud, and we propose a novel learning-based method for RGB-D place-recognition reranking.

\textit{The scarcity of large-scale clean dataset is a notable gap for RGB-D indoor place recognition:} For indoor vision tasks, there are a bunch of datasets designed for object classification, segmentation, etc~\cite{Couprie2013IndoorSS, dai2017scannet, dehghan2021arkitscenes}.
% LOPES2022103489
However, those datasets are not specifically designed for training purposes of RGB-D place recognition tasks, which require positive and negative matched frames by overlaps and large scale for training purposes~\cite{kornilova2023dominating}. HPointLoc~\cite{yudin2022hpointloc} and ScanNet-PR~\cite{cgis} are recently published for RGB-D indoor place recognition tasks, but their matched pairs are selected by the distance of camera poses or point cloud distance instead of the overlap of point clouds. This makes the dataset very noisy because of some nearby point clouds with no overlaps and decreases the efficacy for training learning-based models. To bridge the gap, we introduce two large-scale clean datasets for RGB-D indoor place recognition by choosing frames with overlaps.

\noindent \textbf{Main Results:} In this approach, we aim at the RGB-D indoor place recognition problem. We extend the Context Cluster concept~\cite{cocs} to our approach to process features. The CoCs concept enhances each local feature by the global information of the point cloud, through a cluster and dispatch mechanism. The following describes our contributions. Collectively, the contributions not only push the boundaries of RGB-D indoor place recognition to an integrated retrieval-reranking learning problem but also equip the community with data generation pipeline and new datasets for the task.
\begin{enumerate}
    \item \textbf{New End-to-End Architecture for RGB-D Place Recognition:} 
    We propose Cross-Source-Context Place Recognition (CSCPR) to integrate global retrieval and reranking. We apply the CoCs concept in these two stages to enhance the RGB-D features, especially for reranking, we propose a novel \textit{Self-Context Cluster (SCC)}, which enhances each local feature by global information (all points features).
    \item \textbf{Novel RGB-D Place-recognition Reranking:}  For RGB-D place recognition reranking, besides the SCC model, we present a novel \textit{Cross Source Context Cluster (CSCC)} with a simple correlation calculation to process the local matches between different point clouds for fast and accurate reranking.
    \item \textbf{Curated Large-Scale RGB-D Indoor Place Recognition Datasets:} To address the scarcity of suitable large-scale RGB-D place-recognition datasets, we introduce ARKitIPR and ScanNetIPR RGB-D indoor place recognition task.
    % , specifically designed for training and evaluation purposes of RGB-D indoor place recognition task. 
    We propose a method to generate datasets by point-cloud overlaps. The datasets contain positive and negative frames, keyframes for evaluation, poses and semantic labels of point clouds.
    \item \textbf{Superior Performance Across Multiple Datasets:} We evaluate the performance of CSCPR on different datasets ScanNet-PR~\cite{cgis}, ScanNetIR, and ARKitIPR. As Tab.~\ref{tab:scannetpr_recall} CSCPR achieves at least $36.5\%$ improvement than other SOTA RGB-D indoor place recognition methods in  Recall@1 in the ScanNet-PR. We also achieved at least $43.75\%$ in ScanNetIPR and ARKitIPR. Compared with other place-recognition reranking methods, we improve at least $3.17$ points in the two novel datasets. We demonstrated the effectiveness of our approach in the real-world robot.
\end{enumerate}



\section{Related Work}
\label{sec:related_work}

% place recognition
\noindent 
\textbf{Place Recognition Features and Methods:} Normally, place recognition is handled by calculating the similarities/overlaps between the database and query frames. traditional methods rely on RGB image features, such as SIFT, SURF, BoW,  etc.~\cite{david2004distinctive, cummins2008fab,galvez2012bags, sivic2008efficient}, to compose descriptors for frame matching. 
% For example, ORB~\cite{rublee2011orb} extracts FAST~\cite{rublee2011orb} features and employs BoW to describe and match frames. 
After convolutional networks~\cite{gordo2017end} and attention mechanism~\cite{vaswani2017attention} are proved with better performance in vision tasks, various methods~\cite{gordo2017end, berton2022deep, touvron2021training} are proposed to encode frame features to global descriptors for place recognition, especially, NetVLAD-based methods~\cite{uy2018pointnetvlad, arandjelovic2016netvlad} improve performance by combining convolutions with VLAD cores for global-retrieval. The introduction of Context-of-Clusters (CoCs)~\cite{cocs} offers a computationally efficient yet comparably effective alternative, enhancing local features with global context. Our approach uses this concept to process and aggregate features of RGB-D point clouds.
% Self-Context Cluster (SCC) model adopts the concept for feature processing and aggregates the points to a lower number of centers for place-recognition reranking.

\noindent For RGB-D indoor place recognition tasks, NetVLAD~\cite{arandjelovic2016netvlad}, ORB~\cite{mur2017orb}, etc. use RGB information for place recognition by comparing the global descriptors of images. MinkLoc3D~\cite{komorowski2021minkloc3d} and Point-NetVLAD~\cite{uy2018pointnetvlad} process point clouds, and compare point-cloud global descriptors. CGis-Net~\cite{cgis} applies KP-Conv~\cite{thomas2019kpconv} to encode the geometric information and enhance the features by extracting the semantic information from colors. However, these approaches typically only assess the global descriptors of RGB-D frames. We introduce a novel place-recognition reranking method to improve the accuracy of RGB-D indoor place recognition.

% reranking
\noindent 
\textbf{Place-Recognition Reranking:} The accuracy of place recognition can be enhanced through a subsequent reranking stage following global retrieval~\cite{zhu2023r2former, hausler2021patch, zhang2022rank}. RANSAC-based geometric verification~\cite{vidanapathirana2023spectral, hausler2021patch, wang2022transvpr} is a popular choice for reranking candidates. MAGSAC~\cite{Barath_2020_CVPR} uses a sample method NAPSAC to sample the points and apply a quality function to choose the matched pairs. PatchNet-VLAD~\cite{hausler2021patch} uses RANSAC with scoring methods for reranking after NetVLAD~\cite{arandjelovic2016netvlad}. Although RANSAC focuses on geometric verification, it overlooks non-geometric information. Similarly, registration tasks~\cite{urr, pointmbf, mei2023unsupervised, jiang2023robust, zhang20233d, hatem2023point} also find inliers, but those methods still attempt to match points through geometric verification or rendering without empirically learning frame similarities. Matching methods~\cite{panek2022meshloc, li20232d3d, sarlin2020superglue} like SuperGlue~\cite{sarlin2020superglue} identify inliers of the matching, but cannot guarantee if the frames are overlapped. 
% Thus, learning-based approaches take place in the place recognition and reranking problems by empirically training valuable features for the task. 
Lee et al.~\cite{lee2022correlation} proposed CVNet-Rerank based on convolutional neural networks to process image features and compare the similarities among the features for reranking. R2Former~\cite{zhu2023r2former} used ViTs~\cite{dosovitskiy2020image} to extract the local information of images with higher attention values for reranking. However, those methods are all for RGB place recognition. RGB-D point cloud reranking still relies heavily on RANSAC-based geometric verification, Vidanapathirana et al.~\cite{vidanapathirana2023spectral}, or registration methods, Zhang et al.~\cite{zhang2022rank}. These approaches cannot jointly use color and geometric information effectively. We propose an end-to-end structure to jointly process RGB and geometric information and we also integrate global retrieval and reranking together for RGB-D point cloud place recognition.

\section{Method}
\label{sec:method}
In this section, we first formulate the problem in Section \ref{sec:problem_formulation} and then describe the overall architecture of CSCPR in Section \ref{sec:architecture}, which includes the Self Context Cluster (SCC) and Cross-Source Context Cluster (CSCC) \rev{modules}. Finally, the training strategies are described in Section \ref{sec:training}.


\subsection{Problem Definition}
\label{sec:problem_formulation}

As with other place recognition problems~\cite{liu2023survey, yurtsever2020survey, zhu2023r2former, arandjelovic2016netvlad}, the RGB-D indoor place recognition problem is defined as a point cloud retrieval problem. It's separated into two consecutive tasks, Global Retrieval~\cite{hausler2021patch, uy2018pointnetvlad, arandjelovic2016netvlad, cgis} and Reranking~\cite{zhang2022rank, zhu2023r2former}. In the paper, we use "frame" as an RGB-D colorized point cloud. Denote the place recognition model as $M$. The Global Retrieval calculates the global descriptor $\v_q=M(\Q)$ of a query frame $\Q\in\cq$ and descriptor $\v_d=M(\D)$ of each of the database frames $\D \in \cd$. Then we compare the similarity between $\v_q$ and all $\v_d$ to rank the database frames. \rev{The Reranking re-estimates the similarities based on local features between $\Q$ and $\cd$, and generate a new ranking order}. \rev{The learning objective} is to ensure the similarity between the \rev{($\Q$, $\D_p$)} is much bigger than the similarity between \rev{($\Q$, $\D_n$)}, $s(M(\Q), M(\D_p)) >> s(M(\Q), M(\D_n))$, where $s(\cdot)$ is the similarity function and $\D_p \in \cd$ and $\D_n \in \cd$ correspond to the \rev{positive and negative matches from $\cd$}.

\subsection{Architecture of CSCPR}
\label{sec:architecture}
\begin{figure*}
    \centering
\includegraphics[width=0.9\linewidth]{figs/architecture.png}
    \caption{\textbf{Architecture of CSCPR:} The Blue box indicates Global Retrieval, and the Yellow box represents Reranking. The global retrieval model contains a sequence of layers in the Feature Extractor. The reranking model composes Self Context Clusters (SCC) and a Cross Source Context Cluster (CSCC). After the database frames are ranked by comparing the global descriptors, $\v_q$ and $\v_d$, our reranking stage calculates the relation of local features between query and database frames and aggregates the relation to reranking scores for place recognition.}
    \label{fig:architecture}
    \vspace{-2em}
\end{figure*}

The architecture of CSCPR is shown in Fig.~\ref{fig:architecture}. \rev{It is an end-to-end structure to jointly process the color and geometric information of the frames. It has two modules: the Global Retrieval (blue dash box) and the Reranking (yellow dash box). } The inputs of CSCPR are RGB-D point clouds, $\cp\in \mathcal{R}^{N \times 9}$, where N represents the points number and features include color $\set{r,g,b}$, 3D position $\set{x,y,z}$, and normal vector $\set{n_x,n_y,n_z}$.

The Global Retrieval model calculates the similarities between the query and database frames with their global information (global descriptors) and ranks the database frames. Thus, the critical task of this model is the feature extraction. Recently, CoCs~\cite{cocs} has been proposed with comparable performance to attention mechanism~\cite{vaswani2017attention} but less computational cost. In this project, we apply CoCs structure as the backbone of the Feature Extractor and adapt it from processing RGB to point clouds by changing the reducer layers to PointConvFormer blocks~\cite{wu2023pointconvformer}. We use the Farthest Point Sampling method~\cite{eldar1997farthest} to downsample points and use the K-nearest points as the neighbors to relate the sparse and the dense points for Context Clustering~\cite{cocs}. In the last layer of the Feature Extractor, we aggregate the point features to global descriptors $\v_q$ and $\v_d$ of query and database frames by PointConvFormer. Then cosine similarity is used to measure the similarity between $\v_d$ and $\v_q$. Finally, the database frames are ranked by their similarities. \rev{More details can be found in the Supplement~\ref{sup:global_retrieval}.}


The Global Retrieval model only matches the global descriptors, but some of the local information could be missed. The Reranking model is designed to solve this issue by processing cross-source local features and estimating the similarity score between the query and database frames. There are two critical tasks for designing the Reranking model: 1. The model should be \textbf{fast} and the structure should be light in parameters and computation; 2. The structure should \textbf{effectively process the relation} of the local features from different frames. As shown in Fig.~\ref{fig:scc_cscc}, to satisfy the first criterion, we design a simple structure with only three small but powerful modules. For the second criterion, we propose a novel Cross Source Context Cluster (CSCC) model to process the relation between two frames. The reranking model contains two Self Context Clusters (SCC) and one CSCC. In Fig.~\ref{fig:architecture}, $\f_p^q$ and $\f_p^d$ are the local features of the query and database frames, respectively.


% SCC enhances the local features with the global information of the frame and CSCC processes the cross-source local-feature correlation between the query and database frames. The Reranking model takes the local feature $\f_p$ from the Feature Extractors, as in Fig.~\ref{fig:architecture}. 
% To reduce the computational cost, we choose the local point features after the first CoCs Layer (with more local features than later layers) of the Feature Extractor.


\noindent\textbf{Self Context Cluster (SCC)} performs two functions: 1. To achieve less computational cost, it downsamples the point features to a smaller number of center features. 2. Indoor RGB-D data have large variations w.r.t perspectives, scales, and similar structures for different rooms. SCC learns features from two scales (local fine-scale feature $\f_p$ with denser points from the Feature Extractors in Fig.~\ref{fig:architecture} and coarse-scale feature $\f_c$ with sparser centers) to tackle the challenge. To make the feature more representative, we enhance each of the center features with the global information (all point features) of the frame.
% SCC enhances the coarse-scale features by the local find-scale features w.r.t. the similarities between them. 
% 1. To achieve less computational cost, it downsamples the point features to a smaller number of center features; 
% 2. To make the feature more representative, we enhance each of the center features with the global information (all point features) of the frame.

As shown in the green box of Fig.~\ref{fig:scc_cscc}, inspired by attention mechanism~\cite{vaswani2017attention}, \rev{ we transform the point features by projecting them into two distinct branches in SCC}, reference point feature $\f_p^r$ and source point feature $\f_p^s$:

\begin{align}
    \f_p^r = \norm{l_r(\f_p)}_g \;\;\;\text{and}\;\;\;  \f_c^r = \underset{k}{\text{mean}}(\f_p^r), \\
    \f_p^s = \norm{l_s(\f_p)}_g\;\;\;\text{and}\;\;\; \f_c^s= \underset{k}{\text{mean}}(\f_p^s),
\end{align}
where $l_r$ and $l_s$ are \rev{different} Linear layers to separate the point features to reference and source features. $\norm{\cdot}_g$ represents Group Norm.
The geometric information of the points is used to downsample the points to a smaller number of centers by the Farthest Downsampling method, and we find the K-nearest points for each center and average the neighbors' features to a center feature $\f_c$, where $\f_c^r$ and $\f_c^s$ are reference and source center features. 

The current center features only contain local information about the frame, and we need to enhance it with the frame's global information, which is introduced by all the point features. Thus, we compare each center feature with all point features and aggregate the most globally similar point features to the center. 
% In this function, the global similarity is calculated by the reference features and aggregation is achieved by the source features. 
As in Eq.~\ref{eq:scc_sim}, the global similarity is measured by cosine distance between all $\f_p^r$ and each $\f_c^r$.
\begin{align}
    S = \text{sig} (\alpha \cos{(\f_c^r, \f_p^r)} + \beta),
    \label{eq:scc_sim}
\end{align}
where $\alpha$ and $\beta$ are trainable parameters. $\text{sig}$ and $\cos{}$ are Sigmoid and Cosine Similarity functions. \rev{$\f_p^r \in \mathcal{R}^{N\times D_s}$ and $\f_c^r \in \mathcal{R}^{M\times D_s}$}, where $N>M$ are the numbers of points and centers. $D_s$ is the feature dimension. The similarity matrix is \rev{$S \in \mathcal{R}^{M \times N}$}. To reduce the computational cost, we threshold the similarity matrix by only using the max similar center for each point, and setting other values as 0. 
\rev{To learn the representative multi-scale feature $\Tilde{\f}_c$ for reranking, according to the similarity matrix $S$ from the reference branch, we aggregate the point features to center features in the source branch and normalize them by the similarities}:
\begin{align}
    \Tilde{\f}_{c,i} = \frac{1}{1 + \sum_{j=1}^N \hat{S}_{i,j}}\left(\f_{c,i}^s + \sum_{j=1}^N \hat{S}_{i, j} * \f_{p,j}^s\right)
    \label{eq:aggregation_scc}
\end{align}
\rev{$\f_{p,j}^s$ is the $j_{th}$ vector of $\f_{p}^s$. $\f_{c,i}^s$ is the $i_{th}$ vector of $\f_{c}^s$. } $\hat{S} = \text{Threshold}(S)$ is the similarity matrix after threshold. The final enhanced center feature is $\f_c = l_c(\Tilde{\f_c})$, where $l_c(\cdot)$ is a Linear layer. \rev{As demonstrated in Table~\ref{tab:rerank_ablation}, the learned ”fine-coarse” scale features $\Tilde{\f_c}$ are more effective and efficient than Attention~\cite{vaswani2017attention}, which only processes single-scale features.
}
% Therefore, the top branch learns the relation S between two-scale data. The lower branch learns the representative multi-scale feature $\Tilde{\f}_c$ for reranking by aggregating fine-scale features $\f_p^s$ with coarse features $\f_c^s$ based on S, as shown in Eq.~\ref{eq:aggregation_scc}. 


\noindent\textbf{Cross Source Context Cluster (CSCC)} \rev{captures cross-source correlation between the query and database frames with less computational cost by processing fewer yet representative features and powerful correlation calculations.} 
% processes the correlation of local features between two frames. 
As in the red box (right side) of Fig.~\ref{fig:scc_cscc}, the query and database frames have center features $\f_c^q$ and $\f_c^d$, with shapes of $M_q\times D_c$ and $M_d\times D_c$, where $D_c$ represents the feature dimension and $M_q, M_d$ are center numbers. These sparse center features are the output of SCC, yet those features are representative in terms of multi-modality and multiple-scale information. Besides less features to compute, our correlation computation is also effective:
% . We can calculate the correlation of the center features by:
\begin{align}
    C = \text{sig} (\alpha \cos{(\f_c^q, \f_c^d)} + \beta),
\end{align}
where $\text{sig}$ is the sigmoid function, $\cos$ is the cosine similarity function. $\alpha$ and $\beta$ are trainable parameters. $C \in \crr^{M_q \times M_d}$ is the Correlation matrix. We choose the top $K=500$ center pairs according to the correlation matrix, and other correlation values are masked out as 0. Given the masked correlation, we use it as weights to \rev{concatenate the query and retrieved candidate} features together, where each concatenated feature is $\hat{\f}_{i,j} = l_c( C_{i,j}[\f_{c, i}^q, \f_{c,j}^d])$. $l_c$ represents Linear layers. \rev{Therefore, weighted features from both sources empower the model to learn more effectively.} Finally, the Aggregation function in Fig.~\ref{fig:architecture} only aggregates the most correlated 500 features to one reranking score, $r_s$, as the output of CSCC:
\begin{align}
    &\hat{\f}_c = \frac{1}{1+\mathbf{c}_n}\sum_{j=1}^{M_d} (\frac{1}{1+\mathbf{c}_m}\sum_{i=1}^{M_q} \hat{\f}_{i,j}), \;\; \\
    &\mathbf{c}_m = \sum_{i=1}^{M_q} C_{i,j}, \;\;\mathbf{c}_n = \underset{i}{\text{mean}}(\sum_{j=1}^{M_d} C_{i,j}),
\end{align}
where $\mathbf{c}_m$ is the aggregation of the correlation matrix along the dimension of query center features and $\mathbf{c}_n$ is the aggregation of the correlation matrix along the dimension of database center features and average in the dimension of query center features. Then we have the reranking score of the database point clouds and the query point cloud: $r_s = \text{sig}(l_f(\hat{\f}_c))$,
% \begin{align}
%     r_s = \text{sig}(l_f(\hat{\f}_c))
% \end{align}
where $l_f$ is a Linear layer. Bypassing the feature into a sigmoid function, we generate the reranking score $r_s$ to rerank the candidate database frames. \rev{Our overall design is simple but effective in capturing relationships between two RGB-D clouds (see Table~\ref{tab:rerank_ablation}).}


\begin{figure*}
    \centering
\includegraphics[width=0.9\linewidth]{figs/scc_cscc.png}
    \caption{\textbf{SCC and CSCC:} SCC (left) downsamples the point features $\f_p$ to center features $\f_c$, and enhances $\f_c$ by the similarities with all $\f_p$ in the frame. CSCC calculates the correlation of the local features from these two frames and concatenates the features by the correlation relationship.}
    \label{fig:scc_cscc}
        \vspace{-2em}
\end{figure*}

\subsection{Training}
\label{sec:training}

Training the end-to-end place recognition, CSCPR, requires multiple loss functions for Global Retrieval and Reranking. A cosine annealing scheduler~\cite{loshchilov2016sgdr} and Adam optimizer~\cite{kingma2014adam} are used to schedule the learning rates and the learning rate changes from $10^{-4}$ to $10^{-7}$. For Global Retrieval, We use the Triplet Loss~\cite{schroff2015facenet}, $\cl_t$ as~\cite{liang2024poco}.

% For Global Retrieval, Triplet Loss~\cite{schroff2015facenet} is used: 
% \begin{align}
%     &\cl_t = \max(d(\v_p, \v_q) - \cos(\v_n, \v_q) + m, 0),\;\; \\
%     &d(\cdot) = 1 - \cos(\cdot)
%     \label{eq:triplet}
% \end{align}
% where $\cos{}$ is the cosine similarity function. The margin $m=0.2$. 


For Reranking, given ranked candidates, we need to refine the rank by candidates' local features, so distinguishing between query and hard negatives is crucial in this stage. Therefore, we apply hard negative mining~\cite{robinson2020contrastive} in training and jointly train the two stages together. Since the output similarity $r_s$ is calculated by the Reranking model, we can use the entropy loss function
\begin{equation}
\cl_c = -(y * \log (r_s) + (1-y) * \log(1-r_s))~,
    \label{eq:cross_entropy}
\end{equation}
where $y$ is the label of the matching point clouds. $y=1$ when the point cloud matches the query point cloud, and $y=0$ when they are not matched. The total loss function is $\cl = \beta_t\cl_t + \beta_c \cl_c$, where $\beta_t$ and $\beta_c$ are hyperparameters, and we choose 1.0 in the training.


\section{Dataset Generation}
\label{sec:data_generation}

Most current RGB-D indoor datasets~\cite{sturm12iros, glocker2013real,handa2014benchmark} are designed for classification, segmentation, registration, or rendering tasks, but there are not many large-scale datasets for learning-based RGB-D indoor place recognition. ScanNet-PR~\cite{cgis} is designed for indoor RGB-D place recognition tasks, but because the matching frames are chosen by the distance between point clouds' centers, there is some noise in the dataset. As shown in Figure \ref{fig:dataset_difference} in Supplement~\ref{sec:dataset_differences}, there are cases in which point clouds are very close, but they have no overlaps. If there are no overlapping areas, the model cannot tell whether the two point clouds are in the same place. Therefore, it is also difficult to apply hard negative mining with the ScanNet-PR dataset directly, limiting the final performance of the models. To solve this issue and better evaluate the RGB-D indoor place recognition, we propose two datasets, ScanNetIPR and ARKitIPR, based on ScanNet-V2~\cite{dai2017scannet} and ARKit~\cite{dehghan2021arkitscenes}. The generated ARKitIPR dataset has 4679 scenarios and 377625 frames of point clouds in total. ScanNetIPR has 1605 scenarios and 53201 frames of point clouds in total. Both  datasets contain 1. positive and negative matching frames, 2. the pose of each frame, and 3. database keyframes for the testing datasets. ScanNetIPR also provides semantic labels of the points for segmentation training. The qualitative views of the datasets are in the Supplement Section~\ref{sec:supplement}. Our dataset generation method can also be used in other RGB-D datasets to generate datasets for RGB-D indoor place recognition tasks.

Instead of using distance to build the dataset, because overlap of frames is the major reference for place recognition, in our approach, we use the overlap of point clouds to determine positively or negatively matched cases. There are three steps in the data generation: 1. Choose database frames from the camera's trajectory; 2. Select positive and negative frames for each database frame among all scenarios; 3. Choose the sparse key frames for evaluation. The details of the three steps are in the Supplement~\ref{sup:data_generation}


\begin{table}[!h]
\centering
\begin{tabular}{c|c|ccc}
\textbf{\textit{ScanNet-PR}} & Data Type & R@1 $\uparrow$ &  R@2 $\uparrow$ &  R@3 $\uparrow$\\
\hline
SIFT~\cite{david2004distinctive} + BoW~\cite{sivic2008efficient} & RGB &  16.16 & 21.17 & 24.38 \\
\hline
NetVLAD~\cite{arandjelovic2016netvlad} & RGB &21.77 & 33.81 & 41.49 \\
\hline
PointNetVLAD~\cite{uy2018pointnetvlad} & Point Cloud &27.10 & 32.10 & 37.01 \\
\hline
MinkLoc3D~\cite{komorowski2021minkloc3d} & Point Cloud &15.21 & 19.25 & 22.79 \\
\hline
Indoor DH3D~\cite{du2020dh3d} & RGB-D & 16.10 & 21.92 & 25.30 \\
\hline
CGiS-Net~\cite{cgis} &RGB-D & 61.12 & 70.23 & 75.06 \\
\hline
CGiS-Net w/o color~\cite{cgis} & Point Cloud & 39.62 & 50.92 & 56.14 \\
\hline
\hline
CSCPR$^1$ w/o color & Point Cloud & 44.24 & 55.11 & 60.18\\
\hline
CSCPR w/o color & Point Cloud & 60.58 & 73.59 & 78.29 \\
\hline
CSCPR$^1$ & RGB-D & 64.63 & 75.02 & 80.09 \\\hline
CSCPR & RGB-D & \textbf{84.14} & \textbf{ 89.82} & \textbf{91.25} \\
\end{tabular}
\caption{\textbf{Quantitative Results:} Compared with other state-of-the-art methods, our first stage model (CSCPR$^1$) achieves results comparable to the best of the other methods (CGiS-Net). Our complete model with reranking improved the Recall@1 performance by at least $\mathbf{36.5\%}$.} 
\label{tab:scannetpr_recall}
    \vspace{-2.2em}
% \end{minipage}
% %
% \hspace{0.05\textwidth}
% %
% \begin{minipage}{.45\linewidth}
% \end{minipage}%
\end{table}


\begin{table*}
    \centering
    \begin{tabular}{c| c |c|ccc|ccc} 
   \multirow{2}{*}{Approaches} & \multirow{2}{*}{Data Type}& {Inference}&\multicolumn{3}{c|}{\textit{ARKitIPR}} &\multicolumn{3}{c}{\textit{ScanNetIPR}}  \\ 
    &  & Time (ms) &R@1 $\uparrow$ &  R@2 $\uparrow$ &  R@3 $\uparrow$& R@1 $\uparrow$ &  R@2 $\uparrow$ &  R@3 $\uparrow$\\ \hline 
    CSCPR$^1$                            &RGB-D  & -     & 45.04  & 56.20 & 62.24 & 58.10 & 70.33 & 75.95 \\\hline 
    Kabsch~\cite{arun1987least}          &RGB-D  & 93    & 53.00  & 59.37 & 65.59 & 66.07 & 74.89 & 80.99 \\ \hline
    TEASER~\cite{yang2020teaser}         &RGB-D  & 107   & 56.03  & 62.35 & 66.75 & 69.40 & 80.94 & 82.82 \\ \hline
    R2Former~\cite{zhu2023r2former}      &RGB-D  & 5     & 71.94  & 76.95 & 79.24 & 80.05 & 82.09 & 85.02 \\ \hline
    MAGSAC~\cite{barath2020magsac}       &RGB    & 18    & 20.60  & 33.03 & 38.49 & 41.00 & 47.25 & 52.30 \\ \hline
    SuperGlue~\cite{sarlin2020superglue} &RGB    & 40    & 49.19  & 55.50 & 59.44 & 69.84 & 75.83 & 78.72 \\ \hline
    URR~\cite{urr}                       &RGB-D  & 90    & 31.86  & 40.03 & 46.57 & 46.50 & 56.10 & 62.28 \\ \hline 
    PointMBF~\cite{pointmbf}             &RGB-D  & 300   & 50.12  & 57.30 & 63.47 & 61.27 & 70.92 & 77.40\\ \hline 
    Ours                                 &RGB-D  & 4     & \textbf{75.13} & \textbf{80.24} & \textbf{82.33} & \textbf{83.22} & \textbf{87.76} & \textbf{89.30} \\
    \end{tabular}
    \caption{\textbf{Quantitative Reranking Results:} CSCPR$^1$ is the global retrieval baseline. Compared with other reranking approaches, our place-recognition reranking method outperforms other approaches by at least \textbf{3.19} points in Recall@1.} 
    \label{tab:rerank_recall}
    \vspace{-1em}
\end{table*}


\begin{table*}
    \centering
    \begin{tabular}{c| c |c|ccc|ccc} 
   \multirow{2}{*}{Approaches} & \multirow{2}{*}{Data Type}& {Inference}&\multicolumn{3}{c|}{\textit{ARKitIPR}} &\multicolumn{3}{c}{\textit{ScanNetIPR}}  \\ 
    &  & Time (ms) &R@1 $\uparrow$ &  R@2 $\uparrow$ &  R@3 $\uparrow$& R@1 $\uparrow$ &  R@2 $\uparrow$ &  R@3 $\uparrow$\\ \hline 
    % CSCPR$^1$                            &RGB-D  & -     & 45.04  & 56.20 & 62.24 & 58.10 & 70.33 & 75.95 \\\hline 
    Attention~\cite{vaswani2017attention}&RGB-D  & 11    & 64.14  & 67.65 & 68.81 & 74.95 & 82.94 & 86.22 \\ \hline 
    Ours/SCC                             &RGB-D  & 3     & 65.56  & 68.39 & 69.11 & 76.52 & 80.03 & 81.03 \\ \hline
    Ours/Correlation                     &RGB-D  & 4     & 45.56  & 60.18 & 66.06 & 47.33 & 65.99 & 74.95 \\ \hline
    Ours                                 &RGB-D  & 4     & \textbf{75.13} & \textbf{80.24} & \textbf{82.33} & \textbf{83.22} & \textbf{87.76} & \textbf{89.30} \\
    \end{tabular}
    \caption{\textbf{Reranking Ablation Study:} 
    Ours, Ours/SCC and Ours/Correlation represent our complete reranking, without SCC and without the correlation matrix, respectively. Attention represents the method with a sequence of self-cross attention blocks~\cite{vaswani2017attention}. The table shows effectiveness of our components and the outperformance w.r.t. attention-based alternative by at least $11\%$ in ARKitIPR and ScanNetIPR.} 
    \label{tab:rerank_ablation}
        \vspace{-2.5em}
\end{table*}

\section{Experiment}
\label{sec:experiment}
Our experimental design aims to evaluate the effectiveness and efficiency of our CSCPR against SOTA methods in RGB-D place recognition. To ensure a fair comparison, we conducted training and evaluation across both established dataset, ScanNet-PR, which uses a 3m threshold to select the database frames for place recognition, and also newly proposed datasets, ScanNetIPR and ARKitIPR, which use overlap to select frames. \rev{For each dataset, we perform both training and testing for all models.} The models are trained on 8 Tesla-V100 GPUs, and the input point clouds of CSCPR are constrained to 3000 points by voxelization downsampling. Evaluations are conducted in the device with an NVIDIA RTX A5000 GPU and an Intel Xeon(R) W-2255 CPU. The primary metric used for evaluation is the Recall@k, which \rev{is the percentage of cases where at least one within top-k candidates is positive.} 
% measures the proportion of positive frames within the top k ranked frames when compared to the query frame. 
Our experiments are structured into two distinct evaluations:




\noindent\textbf{E1: End-to-End Solution Evaluation} As mentioned in Section~\ref{sec:intro}, RGB-D indoor place recognition reranking is not well explored and we also did not find any integrated approaches with two stages for RGB-D place recognition. To make a fair comparison, we compare SOTA RGB-D approaches with global retrieval with our CSCPR$^1$ in a public large-scale RGB-D dataset, ScanNet-PR~\cite{cgis}. This experiment also evaluates the performance of new RGB-D point cloud-based datasets. We evaluate both RGB-D and point-cloud approaches in new datasets, ScanNetIPR and ARKtIPR.

\noindent\textbf{E2: Place-Recognition Reranking Evaluation} To make a fair comparison, we compare all the place-recognition reranking approaches with the same Global Retrieval stage. We evaluate the impact of our innovations, SCC and CSCC, on the reranking performance. We quantitatively and qualitatively demonstrate CSCPR's superior reranking performance in terms of accuracy and processing speed, which are our design criteria, than various SOTA approaches. 

% \noindent\textbf{E3: Proposed Dataset Analysis} Fig~\ref{fig:dataset_difference} shows the benefits of our datasets with less noise in the datasets. From the comparison of Tab.~\ref{tab:scannetpr_recall} and \ref{tab:new_scannet} in the Supplement, we observe approaches in our ScanNetIPR have lower recall values than the ScanNet-PR dataset. It means our ScanNetIPR dataset is harder than ScanNet-PR. The reason is using distance to choose database frames leads to more overlapping areas than directly using overlaps among the frames. From Tab.~\ref{tab:new_arkit} and \ref{tab:new_scannet}, we show our new generated datasets are valid for RGB-D indoor place recognition with comparable performance to the results in Tab.~\ref{tab:scannetpr_recall}.

Through this experimental design, we aim to not only validate the performance of CSCPR but also to contribute valuable datasets to the community, facilitating further advancements in RGB-D indoor place recognition.




\noindent\textbf{E1 Results:} In this experiment, we compare our method with SIFT~\cite{david2004distinctive} + BoW~\cite{rublee2011orb}, NetVLAD~\cite{arandjelovic2016netvlad}, PointNetVLAD~\cite{uy2018pointnetvlad}, Indoor DH3D~\cite{du2020dh3d}, MinkLoc3D~\cite{komorowski2021minkloc3d} and CGiS-Net~\cite{cgis} on public large-scale ScanNet-PR dataset. Then we demonstrate our performance on new ScanNetIPR and ARKitIPR. From Tab.~\ref{tab:new_scannet} and \ref{tab:new_arkit} in Supplement, in Recall@1, we observe our global retrieval model (CSCPR$^1$) has 0.5 points improvement in ScanNet-PR, 0.2 points improvement in ScanNetIPR, and around 5 points improvement in ARKitIPR because it is harder with more variety in illumination and density of the point clouds. Our integrated model, CSCPR, has at least $36.5\%$ improvement in ScanNet-PR. We also compare our global retrieval model without color information (CSCPR$^1$ w/o color) with other point-cloud-based approaches and we can observe at least $4.62$ improvement in Tab.~\ref{tab:scannetpr_recall}. The comparisons with novel datasets are in Tab.~\ref{tab:scannetpr_recall} and \ref{tab:new_scannet} in the Supplement.

% It means our ScanNetIPR dataset is harder than ScanNet-PR., because using distance to choose database frames leads to more overlapping areas than using overlaps among the frames directly. 
% {\color{blue} [zhuod]: add more illustrations for overlap metric selection as mentioned in R1-Q2?}


\noindent\textbf{E2 Results (Two sorts of comparisons): } show the benefit of our learning-based place-recognition reranking: 

\noindent\textbf{1. } \textit{Evaluate Place-Recognition Reranking Approaches:} a. classical RANSAC-based geometric verification and b. learning-based place recognition reranking approaches. For a., we implement RGB-based MAGSAC~\cite{barath2020magsac} to fit the homography of images~\cite{hausler2021patch} and RGB-D-based RANSAC + Kabsch~\cite{arun1987least} and TEASER++~\cite{yang2020teaser} for reranking, where Kabsch and TEASER++ calculate the transform of frames and transformed point-cloud distance is used as the geometric verification metric. For b., because of the lack of learning-based place recognition reranking works in RGB-D domain, we adapt the SOTA method, R2Former~\cite{zhu2023r2former}, from RGB domain to RGB-D point space by extending the pixel-position encoding method to $\{x,y,z\}$ positions. As shown in Tab~\ref{tab:rerank_recall}, we observe the learning-based approaches outperform classical approaches, where our method and R2Former outperform classical place-recognition reranking approaches by at least $28\%$. We observe both learning-based and classical RGB-D-based approaches outperform corresponding RGB-based approaches. CSCPR outperforms classical approaches by at least $34\%$ and $20\%$ at Recall@1 in ARKitIPR and ScanNetIPR. Our approach outperforms the adapted R2Former by around 3 points in both datasets at Recall@1. We observe our approach has less inference time than other approaches by at least $20\%$, and this satisfies our design criterion, fast and effective.

\noindent\textbf{2. } \textit{Evaluate Reranking-Similar Methods:} a. Matching and b. registration methods are mostly used for localization~\cite{pointmbf, yang2020teaser, urr}, where given a pair of matched frames, the corresponding features are extracted from overlapped areas and are used to calculate transformation matrices. For a., we use RGB-based SuperGlue~\cite{sarlin2020superglue} and RGB-D-based URR~\cite{urr} to calculate the matching pairs and use the number of matched pairs to determine if the frames are overlapped. For b., besides RANSAC-based geometric verification, we implement PointMBF~\cite{pointmbf} based on calculating the photometric error and location residual error of matched points in the query and database frames. Our method outperforms other reranking-similar approaches by at least $36\%$ on ARKitIPR and ScanNetIPR, as shown in Tab.~\ref{tab:rerank_recall}.

As shown in Fig~\ref{fig:qualitative_results} in Supplement~\ref{sup:qualitative_results}, there are two scenarios. We compare our approach, CSCPR, with the closest place-recognition reranking R2Former and TEASER++. From the bottom two rows in Figure~\ref{fig:qualitative_results}, we see that R2Former can encode semantic information well where it matches the papers on the wall. However, R2Former doesn't balance geometric information effectively; while the overlapped area of the small black trash box is on the left side of the paper, it chooses the point cloud with the wrong positional relations among the door, papers, and the black box. Our approach can handle both color and geometric local information better.



\noindent\textbf{E2 Results (Ablation Study):} As Tab.~\ref{tab:rerank_ablation}, we compare our approach with three different modified versions to highlight the benefits of our design. Attention~\cite{vaswani2017attention} composes a sequence of self-attention and cross-attention models to substitute our SCC and CSCC. Our design based on the CoCs concept outperforms attention-based alternatives by at least $11\%$ on ARKitIPR and ScanNetIPR in Recall@1 and is also faster. SCC improves the performance by at least $9\%$ on the two datasets by enhancing the local features with global information. We also observe the correlation matrix is critical in reranking, and improves by at least $65\%$ on two datasets, as discussed in Section \ref{sec:architecture}, which provides the relationship between two frames. These results demonstrate the effect of our innovative components (SCC and CSCC) and the efficacy of generalizing the CoCs concept to RGB-D point cloud for feature processing in RGB-D place recognition reranking.


\section{Conclusion, Limitations, and Future Work}
% \textbf{Conclusion:} 
We explored the RGB-D place recognition with an integrated mechanism for both global retrieval and reranking. By developing a fast and effective reranking model, we close the gap between RGB-D place recognition reranking and learning-based algorithms. We generalized the CoCs concept to noisy colorized point cloud feature processing and demonstrated better performance in place recognition tasks. We handle the scarcity of RGB-D place recognition datasets and propose a data generation pipeline for the community to explore more datasets. We introduce two large-scale RGB-D datasets for training and testing purposes. We push forward the boundary of RGB-D indoor place recognition accuracy by demonstrating our design outperforming other SOTA approaches by at least $36.5$ in Recall@1 in the ScanNet-PR dataset. For limitations, if the overlapping areas do not have many features, our method may not work well. As part of future work, we would like to apply semantic pretraining to the model to improve its understanding of the environment.

% \textbf{Limitations:} As shown in the Supplementary Section~\ref{sec:supplement}, if the overlapping areas do not have many features, our method may not work well. As part of future work, we would like to apply semantic pretraining to the model to improve its understanding of the environment. Currently, the datasets and training environments used for our evaluations are mostly static, where no time sequential information is provided. However, with sequential frames, if the current observation doesn't have much color or geometric features, more frames would be needed to mitigate the issue and improve the accuracy of place recognition.

==> archive/v2.tex <==
\begin{abstract}
We present a new algorithm, Cross-Source-Context Place Recognition (CSCPR), for RGB-D indoor place recognition that integrates global retrieval and reranking into a single end-to-end model. Unlike prior approaches that primarily focus on the RGB domain, CSCPR is designed to handle the RGB-D data. We extend the Context-of-Clusters (CoCs) for handling noisy colorized point clouds and introduce two novel modules for reranking: the Self-Context Cluster (SCC) and Cross Source Context Cluster (CSCC), which enhance feature representation and match query-database pairs based on local features, respectively. 
We also present two new datasets, ScanNetIPR and ARKitIPR. Our experiments demonstrate that CSCPR significantly outperforms state-of-the-art models on these datasets by at least $36.5\%$ in Recall@1 at ScanNet-PR dataset and $44\%$ in new datasets. Code and datasets will be released.

\end{abstract}

% \keywords{RGB-D Indoor Place Recognition RGB-D datasets}


\section{Introduction}
\label{sec:intro}

Place recognition plays an important role in robotics~\cite{ijcai2021p603, lowry2015visual, liu2023survey, yurtsever2020survey}, {where given query frames the goal is to identify matches from a database that share overlapping field of view with queries based on image similarities}~\cite{kornilova2023dominating, liu2023survey, yurtsever2020survey}. It is used in various applications, such as augmented reality~\cite{middelberg2014scalable}, navigation~\cite{mirowski2018learning, yurtsever2020survey}, SLAM~\cite{yurtsever2020survey, bresson2017simultaneous}, etc. However, the place recognition problem is very challenging~\cite{liu2023survey,yurtsever2020survey, lowry2015visual} due to: (1) different sensors, RGB, RGB-D, Lidar, etc., which require modality-specific feature processing; (2) Environmental challenges, such as illumination changes, dynamic objects, occlusion, and scale variation; (3) RGB-D indoor place recognition is not well studied~\cite{cgis, yurtsever2020survey, lowry2015visual}, where most of the current approaches only use global retrieval for place recognition~\cite{cgis, du2020dh3d}. Our approach focuses on the less explored domain of RGB-D indoor place recognition, and proposes an end-to-end architecture to handle both global retrieval and reranking.



\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{figs/front.jpg}
    \vspace{-1.5em}
    \caption{\textbf{Real-world Experiment:} We propose a novel approach Cross-Source-Context Place Recognition (CSCPR) for RGB-D indoor place recognition. Given a query frame, global retrieval ranks the potentially matched frames, and our novel place-recognition reranking model reranks the candidates to achieve better recognition accuracy.}
    \label{fig:front}
    \vspace{-2em}
\end{figure}


\textit{RGB-D indoor place recognition is not well studied:} 
Visual place recognition has been explored for many years, especially in RGB domain~\cite{lowry2015visual, ijcai2021p603}. However, the potential of RGB-D data is overlooked, especially for indoor environments the depth information can be crucial for place recognition~\cite{cgis, du2020dh3d, lowry2015visual}. Traditional approaches rely on global retrieval, which extracts global descriptors from each frame and ranks the database frames by the similarities with the query frame~\cite{cgis, uy2018pointnetvlad, arandjelovic2016netvlad, yurtsever2020survey}. For RGB-D place recognition, we need to handle different modalities of perceptions (color and geometry), so a good feature extractor is critical in the global retrieval. In recent years, the CoCs~\cite{cocs} method has been proposed and demonstrated with comparable performance with attention mechanism~\cite{vaswani2017attention}, but with different scales of feature processing. In our approach, CSCPR, we take advantage of the concept of CoCs, which uses higher-level global information to enhance local features and propose a novel end-to-end architecture for place recognition jointly integrating both global and local features.

\textit{RGB-D place-recognition reranking is not well studied:} 
% Besides comparing the global descriptors, 
Reranking, as a complement to global retrieval, is to improve the accuracy by evaluating the matches of local features between the query and database frames~\cite{zhu2023r2former, hausler2021patch, vidanapathirana2023spectral}. Therefore, the reranking stage should be fast and accurate in matching local features. The RANSAC-based~\cite{ransac} methods are widely used for reranking by processing the geometric information of query-database frames~\cite{hausler2021patch, vidanapathirana2023spectral}. 
% tan2021instance
However, {RANSAC is not deep-learning-based approach, and cannot be empirically trained to calculate the relationships among all local features}. Recently, learning-based approaches~\cite{zhu2023r2former, lee2022correlation} have been proposed that match empirical local features. However, those approaches are all for RGB-only place recognition. In this work, we generalize the learning-based reranking concept to RGB-D point cloud, and we propose a novel learning-based method for RGB-D place-recognition reranking.

\textit{The scarcity of large-scale clean dataset is a notable gap for RGB-D indoor place recognition:} For indoor vision tasks, there are a bunch of datasets designed for object classification, segmentation, etc~\cite{dai2017scannet, dehghan2021arkitscenes}.
% LOPES2022103489
However, those datasets are not specifically designed for training purposes of RGB-D place recognition tasks, which require positive and negative matched frames by overlaps and large scale for training purposes~\cite{kornilova2023dominating}. HPointLoc~\cite{yudin2022hpointloc} and ScanNet-PR~\cite{cgis} are recently published for RGB-D indoor place recognition tasks, but their matched pairs are selected by the distance of camera poses or point cloud distance instead of the overlap of point clouds. This makes the dataset very noisy because of some nearby point clouds with no overlaps and decreases the efficacy for training learning-based models. To bridge the gap, we introduce two large-scale clean datasets for RGB-D indoor place recognition by choosing frames with overlaps.

\noindent \textbf{Main Results:} In this approach, we aim at the RGB-D indoor place recognition problem. We extend the Context Cluster concept~\cite{cocs} to our approach to process features. {Attention mechanism does not handle the relationship among information from multiple scales of the point cloud. But CoCs concept is capable of handling different scale information by enhancing local features with larger-scale information through a cluster and dispatch mechanism.}  The following describes our contributions. Collectively, the contributions not only push the boundaries of RGB-D indoor place recognition to an integrated retrieval-reranking learning problem but also equip the community with data generation pipeline and new datasets for the task.
\begin{enumerate}
    % \item \textbf{New End-to-End Architecture for RGB-D Place Recognition:} 
    % We propose Cross-Source-Context Place Recognition (CSCPR) to integrate global retrieval and reranking. We apply the CoCs concept in these two stages to enhance the RGB-D features, especially for reranking, we propose a novel \textit{Self-Context Cluster (SCC)}, which enhances each local feature by global information (all points features).
    \item \textbf{Novel RGB-D Place-recognition Reranking:}  For RGB-D place recognition reranking, besides the SCC model, we present a novel \textit{Cross Source Context Cluster (CSCC)} with a simple correlation calculation to process the local matches between different point clouds (sources) for fast and accurate reranking. 
    \item \textbf{Curated Large-Scale RGB-D Indoor Place Recognition Datasets:} To address the scarcity of suitable large-scale RGB-D place-recognition datasets, we introduce ARKitIPR and ScanNetIPR RGB-D indoor place recognition task.
    % , specifically designed for training and evaluation purposes of RGB-D indoor place recognition task. 
    We propose a method to generate datasets by point-cloud overlaps. The datasets contain positive and negative frames, keyframes for evaluation, poses and semantic labels of point clouds.
    \item \textbf{Superior Performance Across Multiple Datasets:} We evaluate the performance of CSCPR on different datasets ScanNet-PR~\cite{cgis}, ScanNetIR, and ARKitIPR. As Tab.~\ref{tab:scannetpr_recall} CSCPR achieves at least $36.5\%$ improvement than other SOTA RGB-D indoor place recognition methods in  Recall@1 in the ScanNet-PR. We also achieved at least $43.75\%$ in ScanNetIPR and ARKitIPR. Compared with other place-recognition reranking methods, we improve at least $3.17$ points in the two novel datasets. We demonstrated the effectiveness of our approach in the real-world robot.
\end{enumerate}



\section{Related Work}
\label{sec:related_work}

% place recognition
\noindent 
\textbf{Place Recognition Features and Methods:} Normally, place recognition is handled by calculating the similarities/overlaps between the database and query frames. traditional methods rely on RGB image features, such as SIFT, SURF, BoW,  etc.~\cite{david2004distinctive, cummins2008fab,galvez2012bags}, to compose descriptors for frame matching. 
% For example, ORB~\cite{rublee2011orb} extracts FAST~\cite{rublee2011orb} features and employs BoW to describe and match frames. 
After convolutional networks~\cite{gordo2017end} and attention mechanism~\cite{vaswani2017attention} are proved with better performance in vision tasks, various methods~\cite{gordo2017end, berton2022deep, touvron2021training} are proposed to encode frame features to global descriptors for place recognition, especially, NetVLAD-based methods~\cite{uy2018pointnetvlad, arandjelovic2016netvlad} improve performance by combining convolutions with VLAD cores for global-retrieval. The introduction of Context-of-Clusters (CoCs)~\cite{cocs} offers a comparably effective alternative but with different scales of feature processing, enhancing local features with global context. Our approach uses this concept to process and aggregate features of RGB-D point clouds.
% Self-Context Cluster (SCC) model adopts the concept for feature processing and aggregates the points to a lower number of centers for place-recognition reranking.

\noindent For RGB-D indoor place recognition tasks, NetVLAD~\cite{arandjelovic2016netvlad}, ORB~\cite{mur2017orb}, etc. use RGB information for place recognition by comparing the global descriptors of images. MinkLoc3D~\cite{komorowski2021minkloc3d} and Point-NetVLAD~\cite{uy2018pointnetvlad} process point clouds, and compare point-cloud global descriptors. CGis-Net~\cite{cgis} applies KP-Conv~\cite{thomas2019kpconv} to encode the geometric information and enhance the features by extracting the semantic information from colors. However, these approaches typically only assess the global descriptors of RGB-D frames. We introduce a novel place-recognition reranking method to improve the accuracy of RGB-D indoor place recognition.

% reranking
\noindent 
\textbf{Place-Recognition Reranking:} The accuracy of place recognition can be enhanced through a subsequent reranking stage following global retrieval~\cite{zhu2023r2former, hausler2021patch, zhang2022rank}. RANSAC-based geometric verification~\cite{vidanapathirana2023spectral, hausler2021patch} is a popular choice for reranking candidates. MAGSAC~\cite{Barath_2020_CVPR} uses a sample method NAPSAC to sample the points and apply a quality function to choose the matched pairs. PatchNet-VLAD~\cite{hausler2021patch} uses RANSAC with scoring methods for reranking after NetVLAD~\cite{arandjelovic2016netvlad}. Although RANSAC focuses on geometric verification, it overlooks non-geometric information. Similarly, registration tasks~\cite{urr, mei2023unsupervised, hatem2023point} also find inliers, but those methods still attempt to match points through geometric verification or rendering without empirically learning frame similarities. Matching methods~\cite{li20232d3d, sarlin2020superglue} like SuperGlue~\cite{sarlin2020superglue} identify inliers of the matching, but cannot guarantee if the frames are overlapped. 
% Thus, learning-based approaches take place in the place recognition and reranking problems by empirically training valuable features for the task. 
Lee et al.~\cite{lee2022correlation} proposed CVNet-Rerank based on convolutional neural networks to process image features and compare the similarities among the features for reranking. R2Former~\cite{zhu2023r2former} used ViTs~\cite{dosovitskiy2020image} to extract the local information of images with higher attention values for reranking. However, those methods are all for RGB place recognition. RGB-D point cloud reranking still relies heavily on RANSAC-based geometric verification, Vidanapathirana et al.~\cite{vidanapathirana2023spectral}, or registration methods, Zhang et al.~\cite{zhang2022rank}. These approaches cannot jointly use color and geometric information effectively. We propose an end-to-end structure to jointly process RGB and geometric information and we also integrate global retrieval and reranking together for RGB-D point cloud place recognition.

\section{Method}
\label{sec:method}
In this section, we first formulate the problem in Section \ref{sec:problem_formulation} and then describe the overall architecture of CSCPR in Section \ref{sec:architecture}, which includes the Self Context Cluster (SCC) and Cross-Source Context Cluster (CSCC) {modules}. Finally, the training strategies are described in Section \ref{sec:training}.


\subsection{Problem Definition}
\label{sec:problem_formulation}

As with other place recognition problems~\cite{liu2023survey, yurtsever2020survey, zhu2023r2former, arandjelovic2016netvlad}, the RGB-D indoor place recognition problem is defined as a point cloud retrieval problem. It's separated into two consecutive tasks, Global Retrieval~\cite{hausler2021patch, uy2018pointnetvlad, arandjelovic2016netvlad, cgis} and Reranking~\cite{zhang2022rank, zhu2023r2former}. In the paper, we use "frame" as an RGB-D colorized point cloud. Denote the place recognition model as $M$. The Global Retrieval calculates the global descriptor $\v_q=M(\Q)$ of a query frame $\Q\in\cq$ and descriptor $\v_d=M(\D)$ of each of the database frames $\D \in \cd$. Then we compare the similarity between $\v_q$ and all $\v_d$ to rank the database frames. {The Reranking re-estimates the similarities based on local features between $\Q$ and $\cd$, and generate a new ranking order}. {The learning objective} is to ensure the similarity between the {($\Q$, $\D_p$)} is much bigger than the similarity between {($\Q$, $\D_n$)}, $s(M(\Q), M(\D_p)) >> s(M(\Q), M(\D_n))$, where $s(\cdot)$ is the similarity function and $\D_p \in \cd$ and $\D_n \in \cd$ correspond to the {positive and negative matches from $\cd$}.

\subsection{Architecture of CSCPR}
\label{sec:architecture}
\begin{figure*}
    \centering
\includegraphics[width=0.9\linewidth]{figs/architecture.png}
    \vspace{-0.5em}
    \caption{\textbf{Architecture of CSCPR:} The Blue box indicates Global Retrieval, and the Yellow box represents Reranking. The global retrieval model contains a sequence of layers in the Feature Extractor. The reranking model composes Self Context Clusters (SCC) and a Cross Source Context Cluster (CSCC). After the database frames are ranked by comparing the global descriptors, $\v_q$ and $\v_d$, our reranking stage calculates the relation of local features between query and database frames and aggregates the relation to reranking scores for place recognition.}
    \label{fig:architecture}
    \vspace{-2em}
\end{figure*}

The architecture of CSCPR is shown in Fig.~\ref{fig:architecture}. {It is an end-to-end structure to jointly process the color and geometric information of the frames. It has two modules: the Global Retrieval (blue dash box) and the Reranking (yellow dash box). } The inputs of CSCPR are RGB-D point clouds, $\cp\in \mathcal{R}^{N \times 9}$, where N represents the points number and features include color $\set{r,g,b}$, 3D position $\set{x,y,z}$, and normal vector $\set{n_x,n_y,n_z}$.  {Global retrieval is from our previous work~\cite{liang2024poco}, which uses CoCs to calculate the global descriptor of the RGB-D point cloud. }

However, the Global Retrieval model only matches the global descriptors, but some of the local information could be missed. The Reranking model is designed to solve this issue by processing cross-source local features and estimating the similarity score between the query and database frames. There are two critical tasks for designing the Reranking model: 1. The model should be \textbf{fast} and the structure should be light in parameters and computation; 2. The structure should \textbf{effectively process the relation} of the local features from different frames. As shown in Fig.~\ref{fig:scc_cscc}, to satisfy the first criterion, we design a simple structure with only three small but powerful modules. For the second criterion, we propose a novel Cross Source Context Cluster (CSCC) model to process the relation between two frames. The reranking model contains two Self Context Clusters (SCC) and one CSCC. In Fig.~\ref{fig:architecture}, $\f_p^q$ and $\f_p^d$ are the local features of the query and database frames, respectively.

\noindent\textbf{Self Context Cluster (SCC)} performs two functions: 1. To achieve less memory usage and multiple scale feature processing, it downsamples the point features to a smaller number of center features. 2. Indoor RGB-D data have large variations w.r.t perspectives, scales, and similar structures for different rooms. SCC learns features from two scales (local fine-scale feature $\f_p$ with denser points from the Feature Extractors in Fig.~\ref{fig:architecture} and coarse-scale feature $\f_c$ with sparser centers) to tackle the challenge. To make the feature more representative, we enhance each of the center features with the global information (all point features) of the frame.


As shown in the green box of Fig.~\ref{fig:scc_cscc}, inspired by attention mechanism~\cite{vaswani2017attention}, { we transform the point features by projecting them into two distinct branches in SCC}, reference point feature $\f_p^r$ and source point feature $\f_p^s$:

\begin{align}
    \f_p^r = \norm{l_r(\f_p)}_g \;\;\;\text{and}\;\;\;  \f_c^r = \underset{k}{\text{mean}}(\f_p^r), \\
    \f_p^s = \norm{l_s(\f_p)}_g\;\;\;\text{and}\;\;\; \f_c^s= \underset{k}{\text{mean}}(\f_p^s),
\end{align}
where $l_r$ and $l_s$ are {different} Linear layers to separate the point features to reference and source features. $\norm{\cdot}_g$ represents Group Norm.
The geometric information of the points is used to downsample the points to a smaller number of centers by the Farthest Downsampling method, and we find the K-nearest points for each center and average the neighbors' features to a center feature $\f_c$, where $\f_c^r$ and $\f_c^s$ are reference and source center features. 

The current center features only contain local information about the frame, and we need to enhance it with the frame's global information, which is introduced by all the point features. Thus, we compare each center feature with all point features and aggregate the most globally similar point features to the center. 
% In this function, the global similarity is calculated by the reference features and aggregation is achieved by the source features. 
As in Eq.~\ref{eq:scc_sim}, the global similarity is measured by cosine distance between all $\f_p^r$ and each $\f_c^r$.
\begin{align}
    S = \text{sig} (\alpha \cos{(\f_c^r, \f_p^r)} + \beta),
    \label{eq:scc_sim}
\end{align}
where $\alpha$ and $\beta$ are trainable parameters. $\text{sig}$ and $\cos{}$ are Sigmoid and Cosine Similarity functions. {$\f_p^r \in \mathcal{R}^{N\times D_s}$ and $\f_c^r \in \mathcal{R}^{M\times D_s}$}, where $N>M$ are the numbers of points and centers. $D_s$ is the feature dimension. The similarity matrix is {$S \in \mathcal{R}^{M \times N}$}. We threshold the similarity matrix by only using the max similar center for each point, and setting other values as 0. 
{To learn the representative multi-scale feature $\Tilde{\f}_c$ for reranking, according to the similarity matrix $S$ from the reference branch, we aggregate the point features to center features in the source branch and normalize them by the similarities}:
\begin{align}
    \Tilde{\f}_{c,i} = \frac{1}{1 + \sum_{j=1}^N \hat{S}_{i,j}}\left(\f_{c,i}^s + \sum_{j=1}^N \hat{S}_{i, j} * \f_{p,j}^s\right)
    \label{eq:aggregation_scc}
\end{align}
{$\f_{p,j}^s$ is the $j_{th}$ vector of $\f_{p}^s$. $\f_{c,i}^s$ is the $i_{th}$ vector of $\f_{c}^s$. } $\hat{S} = \text{Threshold}(S)$ is the similarity matrix after threshold. The final enhanced center feature is $\f_c = l_c(\Tilde{\f_c})$, where $l_c(\cdot)$ is a Linear layer. {As demonstrated in Table~\ref{tab:rerank_ablation}, the learned ”fine-coarse” scale features $\Tilde{\f_c}$ are more effective and efficient than Attention~\cite{vaswani2017attention}, which only processes single-scale features.
}
% Therefore, the top branch learns the relation S between two-scale data. The lower branch learns the representative multi-scale feature $\Tilde{\f}_c$ for reranking by aggregating fine-scale features $\f_p^s$ with coarse features $\f_c^s$ based on S, as shown in Eq.~\ref{eq:aggregation_scc}. 


\noindent\textbf{Cross Source Context Cluster (CSCC)} {captures cross-source correlation between the query and database frames with less points by processing fewer yet representative features and powerful correlation calculations.} 
% processes the correlation of local features between two frames. 
As in the red box (right side) of Fig.~\ref{fig:scc_cscc}, the query and database frames have center features $\f_c^q$ and $\f_c^d$, with shapes of $M_q\times D_c$ and $M_d\times D_c$, where $D_c$ represents the feature dimension and $M_q, M_d$ are center numbers. These sparse center features are the output of SCC, yet those features are representative in terms of multi-modality and multiple-scale information.  {To calculate the correlation of the two point sources, we use the same calculation method as Eq.~\ref{eq:scc_sim} but with the same scale of points, $C = \text{sig} (\alpha \cos{(\f_c^q, \f_c^d)} + \beta)$.}

% Besides less features to compute, our correlation computation is also effective:
% . We can calculate the correlation of the center features by:
where $\text{sig}$ is the sigmoid function, $\cos$ is the cosine similarity function. $\alpha$ and $\beta$ are trainable parameters. $C \in \crr^{M_q \times M_d}$ is the Correlation matrix. We choose the top $K=500$ center pairs according to the correlation matrix, and other correlation values are masked out as 0. Given the masked correlation, we use it as weights to {concatenate the query and retrieved candidate} features together, where each concatenated feature is $\hat{\f}_{i,j} = l_c( C_{i,j}[\f_{c, i}^q, \f_{c,j}^d])$. $l_c$ represents Linear layers. {Therefore, weighted features from both sources empower the model to learn more effectively.} Finally, the Aggregation function in Fig.~\ref{fig:architecture} only aggregates the most correlated 500 features to one reranking score, $r_s$, as the output of CSCC:
\begin{align}
    &\hat{\f}_c = \frac{1}{1+\mathbf{c}_n}\sum_{j=1}^{M_d} (\frac{1}{1+\mathbf{c}_m}\sum_{i=1}^{M_q} \hat{\f}_{i,j}), \;\; \\
    &\mathbf{c}_m = \sum_{i=1}^{M_q} C_{i,j}, \;\;\mathbf{c}_n = \underset{i}{\text{mean}}(\sum_{j=1}^{M_d} C_{i,j}),
\end{align}
where $\mathbf{c}_m$ is the aggregation of the correlation matrix along the dimension of query center features and $\mathbf{c}_n$ is the aggregation of the correlation matrix along the dimension of database center features and average in the dimension of query center features. Then we have the reranking score of the database point clouds and the query point cloud: $r_s = \text{sig}(l_f(\hat{\f}_c))$,
% \begin{align}
%     r_s = \text{sig}(l_f(\hat{\f}_c))
% \end{align}
where $l_f$ is a Linear layer. Bypassing the feature into a sigmoid function, we generate the reranking score $r_s$ to rerank the candidate database frames. {Our overall design is simple but effective in capturing relationships between two RGB-D clouds (see Table~\ref{tab:rerank_ablation}).}


\begin{figure*}
    \centering
\includegraphics[width=0.9\linewidth]{figs/scc_cscc.png}
    \vspace{-0.5em}
    \caption{\textbf{SCC and CSCC:} SCC (left) downsamples the point features $\f_p$ to center features $\f_c$, and enhances $\f_c$ by the similarities with all $\f_p$ in the frame. CSCC calculates the correlation of the local features from these two frames and concatenates the features by the correlation relationship.}
    \label{fig:scc_cscc}
        \vspace{-2em}
\end{figure*}

\subsection{Training}
\label{sec:training}

Training the end-to-end place recognition, CSCPR, requires multiple loss functions for Global Retrieval and Reranking. A cosine annealing scheduler~\cite{loshchilov2016sgdr} and Adam optimizer~\cite{kingma2014adam} are used to schedule the learning rates and the learning rate changes from $10^{-4}$ to $10^{-7}$. For Global Retrieval, We use the Triplet Loss~\cite{schroff2015facenet}, $\cl_t$ as~\cite{liang2024poco}.


For Reranking, given ranked candidates, we need to refine the rank by candidates' local features, so distinguishing between query and hard negatives is crucial in this stage. Therefore, we apply hard negative mining~\cite{robinson2020contrastive} in training and jointly train the two stages together. Since the output similarity $r_s$ is calculated by the Reranking model, we can use the entropy loss function
\begin{equation}
\cl_c = -(y * \log (r_s) + (1-y) * \log(1-r_s))~,
    \label{eq:cross_entropy}
\end{equation}
where $y$ is the label of the matching point clouds. $y=1$ when the point cloud matches the query point cloud, and $y=0$ when they are not matched. The total loss function is $\cl = \beta_t\cl_t + \beta_c \cl_c$, where $\beta_t$ and $\beta_c$ are hyperparameters, and we choose 1.0 in the training.


\section{Dataset Generation}
\label{sec:data_generation}

Most current RGB-D indoor datasets~\cite{sturm12iros, glocker2013real,handa2014benchmark} are designed for classification, segmentation, registration, or rendering tasks, but there are not many large-scale datasets for learning-based RGB-D indoor place recognition. ScanNet-PR~\cite{cgis} is designed for indoor RGB-D place recognition tasks, but because the matching frames are chosen by the distance between point clouds' centers, there is some noise in the dataset. As shown in Figure \ref{fig:dataset_difference} in Supplement~\ref{sec:dataset_differences}, there are cases in which point clouds are very close, but they have no overlaps. If there are no overlapping areas, the model cannot tell whether the two point clouds are in the same place. Therefore, it is also difficult to apply hard negative mining with the ScanNet-PR dataset directly, limiting the final performance of the models. To solve this issue and better evaluate the RGB-D indoor place recognition, we propose two datasets, ScanNetIPR and ARKitIPR, based on ScanNet-V2~\cite{dai2017scannet} and ARKit~\cite{dehghan2021arkitscenes}. The generated ARKitIPR dataset has 4679 scenarios and 377625 frames of point clouds in total. ScanNetIPR has 1605 scenarios and 53201 frames of point clouds in total. Both  datasets contain 1. positive and negative matching frames, 2. the pose of each frame, 3. database keyframes for the testing datasets and for recall calculation, and 4. each point cloud contains positional $x,y,z$, normal $n_x,n_y,n_z$, and color $r,g,b$ information. ScanNetIPR also provides semantic labels of the points for segmentation training. The qualitative views of the datasets are in Figure \ref{fig:dataset_diff} in the Supplement Section~\ref{sec:supplement}. Our dataset generation method can also be used in other RGB-D datasets to generate datasets for RGB-D indoor place recognition tasks.


\vspace{-1em}
\begin{algorithm}
\caption{The frames are chosen by the motion of the camera, where we use an overlap threshold to select the representative frames for place recognition tasks. The FrameOverlap() function is as Eq.~\ref{eq:frame_overlap}.}
\begin{algorithmic}
\Require $N$ consecutive frames, 
\Require $F_l \gets \{ \P_0, p_0 \}$
\Require database = $\{F_l, \}$
\While{$n < N$}
\State $F_n \gets \{ \P_n, p_n \}$
\If{FrameOverlap($F_l$, $F_n$) $< T_c$ }
    \State database.add($F_n$)
    \State $F_l = F_n$
\EndIf
\EndWhile
\end{algorithmic}
\label{alg:choose_database}
\end{algorithm}
\vspace{-1em}

 {Instead of using distance to build the dataset, because overlap of frames is the major reference for place recognition, in our approach, we use the overlap of point clouds to determine positively or negatively matched cases. The algorithm generating training data is as Algorithm~\ref{alg:choose_database}:

The first step is to generate frames according to the motion of the camera. In contrast to the odometry tasks, place recognition does not require lots of very similar point clouds to estimate the transformation matrices, because those point clouds do not provide much different information for place retrieval and add burdens for training. Therefore, the frames are chosen by some overlap threshold along the trajectory of the camera motion, where if the current frame overlaps too much with the last frame it will be dropped, as shown in Algorithm \ref{alg:choose_database}. The overlap in this step is calculated by the symmetric intersection of the union (IoU) of the voxelized point clouds:
\begin{align}
    &[\v_n, \v_l] = 
    \text{voxelize}([p_n \P_n, \;p_l \P_l]), \;\;\; \\
    &\text{FrameOverlap}{(\P_n, \P_l)} = \frac{\abs{v_n \bigcap v_l}}{\abs{v_n \bigcup v_l}}
    \label{eq:frame_overlap}
\end{align}
$\P_n$ and $\P_l$ are points chosen by frustums in the integrated point cloud of the scenario. $\v_n$ and $\v_l$ are the voxels of the $n_{th}$ frame and the last selected frame, respectively. $p_n \P_n$ represents the point cloud transformed in the global frame. The threshold $T_c = 0.5$ is used in the data generation task.

The second step is to choose the positive frames in the same scenario and negative cases in all scenarios. Since this step treats each frame as a query frame to calculate the overlap with other frames in the scenario, the overlap is mostly w.r.t. the query frame. Therefore, an asymmetric overlap metric can be used
\begin{align}
    &\text{Overlap}{(\P_q, \P_d)} = \frac{\abs{v_q \bigcap v_o}}{\abs{v_q}}, \;\; \\
    &\v_q=\text{voxelize}(\P_q), \;\; \v_d=\text{voxelize}(\P_d)
\end{align}
where $\P_q$ and $\P_d$ are query and database point clouds. $\v_q$ and $\v_d$ are the voxels of these two point clouds. Then the positive frames are selected by the threshold $\text{Overlap} > T_p$. Negative frames can be selected by $\text{Overlap} <= T_n$. Normally, the negative threshold $T_n=0$.

The third step is to extract the key frames of each scenario, where we build a graph for each scenario using the positively matched frames and choose the dominating nodes as the keyframes of the scenario as \cite{kornilova2023dominating}, according to the connection of the graph.}


% \vspace{-1em}



\begin{table*}
    \centering
    \begin{tabular}{c| c |c|ccc|ccc} 
   \multirow{2}{*}{Approaches} & \multirow{2}{*}{Data Type}& {Inference}&\multicolumn{3}{c|}{\textit{ARKitIPR}} &\multicolumn{3}{c}{\textit{ScanNetIPR}}  \\ 
    &  & Time (ms) &R@1 $\uparrow$ &  R@2 $\uparrow$ &  R@3 $\uparrow$& R@1 $\uparrow$ &  R@2 $\uparrow$ &  R@3 $\uparrow$\\ \hline 
    CSCPR$^1$                            &RGB-D  & -     & 45.12  & 57.10 & 62.14 & 58.10 & 70.33 & 75.95 \\\hline 
    Kabsch~\cite{arun1987least}          &RGB-D  & 93    & 53.00  & 59.37 & 65.59 & 66.07 & 74.89 & 80.99 \\ \hline
    TEASER~\cite{yang2020teaser}         &RGB-D  & 107   & 56.03  & 62.35 & 66.75 & 69.40 & 80.94 & 82.82 \\ \hline
    R2Former~\cite{zhu2023r2former}      &RGB-D  & 5     & 71.94  & 76.95 & 79.24 & 80.05 & 82.09 & 85.02 \\ \hline
    MAGSAC~\cite{barath2020magsac}       &RGB    & 18    & 20.60  & 33.03 & 38.49 & 41.00 & 47.25 & 52.30 \\ \hline
    SuperGlue~\cite{sarlin2020superglue} &RGB    & 40    & 49.19  & 55.50 & 59.44 & 69.84 & 75.83 & 78.72 \\ \hline
    SelaVPR~\cite{lu2024towards}         &RGB    & 11.4    &  56.32 & 63.81 & 67.56 & 67.31  & 76.47 & 80.60 \\ \hline
    URR~\cite{urr}                       &RGB-D  & 90    & 31.86  & 40.03 & 46.57 & 46.50 & 56.10 & 62.28 \\ \hline 
    PointMBF~\cite{pointmbf}             &RGB-D  & 300   & 50.12  & 57.30 & 63.47 & 61.27 & 70.92 & 77.40\\ \hline 
    Ours                                 &RGB-D  & 4     & \textbf{75.13} & \textbf{80.24} & \textbf{82.33} & \textbf{83.22} & \textbf{87.76} & \textbf{89.30} \\
    \end{tabular}
    \vspace{-0.5em}
    \caption{\textbf{Quantitative Reranking Results:} CSCPR$^1$ is the global retrieval baseline. Compared with other reranking approaches, our place-recognition reranking method outperforms other approaches by at least \textbf{3.19} points in Recall@1.} 
    \label{tab:rerank_recall}
    \vspace{-1em}
\end{table*}


\begin{table*}
    \centering
    \begin{tabular}{c| c |c|ccc|ccc} 
   \multirow{2}{*}{Approaches} & \multirow{2}{*}{Data Type}& {Inference}&\multicolumn{3}{c|}{\textit{ARKitIPR}} &\multicolumn{3}{c}{\textit{ScanNetIPR}}  \\ 
    &  & Time (ms) &R@1 $\uparrow$ &  R@2 $\uparrow$ &  R@3 $\uparrow$& R@1 $\uparrow$ &  R@2 $\uparrow$ &  R@3 $\uparrow$\\ \hline 
    % CSCPR$^1$                            &RGB-D  & -     & 45.04  & 56.20 & 62.24 & 58.10 & 70.33 & 75.95 \\\hline 
    Attention~\cite{vaswani2017attention}&RGB-D  & 11    & 64.14  & 67.65 & 68.81 & 74.95 & 82.94 & 86.22 \\ \hline 
    Ours/SCC                             &RGB-D  & 3     & 65.56  & 68.39 & 69.11 & 76.52 & 80.03 & 81.03 \\ \hline
    Ours/Correlation                     &RGB-D  & 4     & 45.56  & 60.18 & 66.06 & 47.33 & 65.99 & 74.95 \\ \hline
    Ours                                 &RGB-D  & 4     & \textbf{75.13} & \textbf{80.24} & \textbf{82.33} & \textbf{83.22} & \textbf{87.76} & \textbf{89.30} \\
    \end{tabular}
    \vspace{-0.5em}
    \caption{\textbf{Reranking Ablation Study:} 
    Ours, Ours/SCC and Ours/Correlation represent our complete reranking, without SCC and without the correlation matrix, respectively. Attention represents the method with a sequence of self-cross attention blocks~\cite{vaswani2017attention}. The table shows effectiveness of our components and the outperformance w.r.t. attention-based alternative by at least $11\%$ in ARKitIPR and ScanNetIPR.} 
    \label{tab:rerank_ablation}
        \vspace{-2.5em}
\end{table*}

\section{Experiment}
\label{sec:experiment}
Our experimental design aims to evaluate the effectiveness and efficiency of our CSCPR against SOTA methods in RGB-D place recognition. To ensure a fair comparison, we conducted training and evaluation across both established dataset, ScanNet-PR, which uses a 3m threshold to select the database frames for place recognition, and also newly proposed datasets, ScanNetIPR and ARKitIPR, which use overlap to select frames. {For each dataset, we perform both training and testing for all models.} The models are trained on 8 Tesla-V100 GPUs, and the input point clouds of CSCPR are constrained to 3000 points by voxelization downsampling. Evaluations are conducted in the device with an NVIDIA RTX A5000 GPU and an Intel Xeon(R) W-2255 CPU. The primary metric used for evaluation is the  {Recall@1-3}, which {is the percentage of cases where at least one within top-k candidates is positive.} Our experiments are structured into three distinct evaluations:

\noindent\textbf{E1: End-to-End Solution Evaluation} As mentioned in Section~\ref{sec:intro}, RGB-D indoor place recognition reranking is not well explored and we also did not find any integrated approaches with two stages for RGB-D place recognition. To make a fair comparison, we compare SOTA RGB-D approaches with global retrieval with our CSCPR$^1$ (PoCo)~\cite{liang2024poco} and full CSCPR in a public large-scale RGB-D dataset, ScanNet-PR~\cite{cgis} as shown in the Section \ref{sec:sup_pr_results}. This experiment also evaluates the performance of new RGB-D point cloud-based datasets. We evaluate both RGB-D and point-cloud approaches in new datasets, ScanNetIPR and ARKtIPR.
\begin{table}[!h]
\centering
\begin{tabular}{c|c|ccc}
\textbf{\textit{ScanNet-PR}} & Data Type & R@1 $\uparrow$ &  R@2 $\uparrow$ &  R@3 $\uparrow$\\
\hline
SIFT~\cite{david2004distinctive} + BoW~\cite{sivic2008efficient} & RGB &  16.16 & 21.17 & 24.38 \\
\hline
NetVLAD~\cite{arandjelovic2016netvlad} & RGB &21.77 & 33.81 & 41.49 \\
\hline
PointNetVLAD~\cite{uy2018pointnetvlad} & Point Cloud &27.10 & 32.10 & 37.01 \\
\hline
MinkLoc3D~\cite{komorowski2021minkloc3d} & Point Cloud &15.21 & 19.25 & 22.79 \\
\hline
Indoor DH3D~\cite{du2020dh3d} & RGB-D & 16.10 & 21.92 & 25.30 \\
\hline
CGiS-Net~\cite{cgis} &RGB-D & 61.12 & 70.23 & 75.06 \\
\hline
PoCo~\cite{liang2024poco} & RGB-D & 64.63 & 75.02 & 80.09 \\\hline
AEGIS-NET~\cite{ming2024aegis} & RGB-D & 65.09 & 74.26 & 79.06 \\
\hline
CGiS-Net w/o color~\cite{cgis} & Point Cloud & 39.62 & 50.92 & 56.14 \\
\hline
PoCo~\cite{liang2024poco} w/o color & Point Cloud & 44.34 & 54.27 & 59.78\\
\hline
\hline
CSCPR w/o color & Point Cloud & 60.58 & 73.59 & 78.29 \\
\hline
CSCPR & RGB-D & \textbf{84.14} & \textbf{ 89.82} & \textbf{91.25} \\
\end{tabular}
\caption{\textbf{Quantitative Results:} Compared with other state-of-the-art methods, our first stage model (CSCPR$^1$) achieves results comparable to the best of the other methods (CGiS-Net). Our complete model with reranking improved the Recall@1 performance by at least $\mathbf{36.5\%}$.} 
\label{tab:scannetpr_recall}
    \vspace{-2.2em}
\end{table}
\noindent\textbf{E2: Proposed Dataset Analysis} Fig~\ref{fig:dataset_difference} shows the benefits of our datasets with less noise in the datasets. From the comparison of Tab.~\ref{tab:scannetpr_recall} and \ref{tab:new_scannet} in the Supplement, we observe approaches in our ScanNetIPR have lower recall values than the ScanNet-PR dataset. It means our ScanNetIPR dataset is harder than ScanNet-PR. The reason is using distance to choose database frames leads to more overlapping areas than directly using overlaps among the frames. From Tab.~\ref{tab:new_arkit} and \ref{tab:new_scannet}, we show our new generated datasets are valid for RGB-D indoor place recognition with comparable performance to the results in Tab.~\ref{tab:scannetpr_recall}. Through this experimental design, we aim to not only validate the performance of CSCPR but also to contribute valuable datasets to the community, facilitating further advancements in RGB-D indoor place recognition.

 {\noindent\textbf{E3: Place-Recognition Reranking Evaluation}} To make a fair comparison, we compare all the place-recognition reranking approaches with the same Global Retrieval stage. We evaluate the impact of our innovations, SCC and CSCC, on the reranking performance. We quantitatively and qualitatively demonstrate CSCPR's superior reranking performance in terms of accuracy and processing speed, which are our design criteria, than various SOTA approaches. 

 {\noindent\textbf{Comparisons with other Reranking approaches: } a. classical RANSAC-based geometric verification, b. learning-based place recognition reranking approaches. c. matching methods, and d. registration methods~\cite{pointmbf, yang2020teaser, urr}, which are mostly used for localization, where given a pair of matched frames, the corresponding features are extracted from overlapped areas and are used to calculate transformation matrices. For a., we implement RGB-based MAGSAC~\cite{barath2020magsac} to fit the homography of images~\cite{hausler2021patch} and RGB-D-based RANSAC + Kabsch~\cite{arun1987least} for reranking. For b., because of the lack of learning-based place recognition reranking works in RGB-D domain, we adapt the SOTA method, R2Former~\cite{zhu2023r2former}, from RGB domain to RGB-D point space by extending the pixel-position encoding method to $\{x,y,z\}$ positions. For c., we use RGB-based SuperGlue~\cite{sarlin2020superglue} and RGB-D-based URR~\cite{urr} to calculate the matching pairs and use the number of matched pairs to determine if the frames are overlapped. For d., we compared with TEASER++~\cite{yang2020teaser} and we implement PointMBF~\cite{pointmbf} based on calculating the photometric error and location residual error of matched points in the query and database frames.

As shown in Tab~\ref{tab:rerank_recall}, we observe the learning-based approaches outperform RANSAC-based approaches and both RGB-D-based approaches outperform corresponding RGB-based approaches. Our approach outperforms both learning-based and RANSAC-based approaches. Specifically, CSCPR outperforms RANSAC-based approaches by at least $34\%$ and $20\%$ at Recall@1 in ARKitIPR and ScanNetIPR. Our approach outperforms the adapted R2Former by around 3 points in both datasets at Recall@1. Our method outperforms other matching and registration approaches by at least $36\%$ on ARKitIPR and ScanNetIPR, as shown in Tab.~\ref{tab:rerank_recall}. We also observe our approach has less inference time than other approaches by at least $20\%$, and this satisfies our design criterion, fast and effective. }

% \noindent\textbf{1. } \textit{Evaluate Place-Recognition Reranking Approaches:} a. classical RANSAC-based geometric verification and b. learning-based place recognition reranking approaches. For a., we implement RGB-based MAGSAC~\cite{barath2020magsac} to fit the homography of images~\cite{hausler2021patch} and RGB-D-based RANSAC + Kabsch~\cite{arun1987least} and TEASER++~\cite{yang2020teaser} for reranking, where Kabsch and TEASER++ calculate the transform of frames and transformed point-cloud distance is used as the geometric verification metric. For b., because of the lack of learning-based place recognition reranking works in RGB-D domain, we adapt the SOTA method, R2Former~\cite{zhu2023r2former}, from RGB domain to RGB-D point space by extending the pixel-position encoding method to $\{x,y,z\}$ positions. As shown in Tab~\ref{tab:rerank_recall}, we observe the learning-based approaches outperform classical approaches, where our method and R2Former outperform classical place-recognition reranking approaches by at least $28\%$. We observe both learning-based and classical RGB-D-based approaches outperform corresponding RGB-based approaches. CSCPR outperforms classical approaches by at least $34\%$ and $20\%$ at Recall@1 in ARKitIPR and ScanNetIPR. Our approach outperforms the adapted R2Former by around 3 points in both datasets at Recall@1. We observe our approach has less inference time than other approaches by at least $20\%$, and this satisfies our design criterion, fast and effective.

% \noindent\textbf{2. } \textit{Evaluate Reranking-Similar Methods:} a. Matching and b. registration methods are mostly used for localization~\cite{pointmbf, yang2020teaser, urr}, where given a pair of matched frames, the corresponding features are extracted from overlapped areas and are used to calculate transformation matrices. For a., we use RGB-based SuperGlue~\cite{sarlin2020superglue} and RGB-D-based URR~\cite{urr} to calculate the matching pairs and use the number of matched pairs to determine if the frames are overlapped. For b., besides RANSAC-based geometric verification, we implement PointMBF~\cite{pointmbf} based on calculating the photometric error and location residual error of matched points in the query and database frames. Our method outperforms other reranking-similar approaches by at least $36\%$ on ARKitIPR and ScanNetIPR, as shown in Tab.~\ref{tab:rerank_recall}.

As shown in Fig~\ref{fig:qualitative_results} in Supplement~\ref{sup:qualitative_results}, there are two scenarios. We compare our approach, CSCPR, with the closest place-recognition reranking R2Former and TEASER++. From the bottom two rows in Figure~\ref{fig:qualitative_results}, we see that R2Former can encode semantic information well where it matches the papers on the wall. However, R2Former doesn't balance geometric information effectively; while the overlapped area of the small black trash box is on the left side of the paper, it chooses the point cloud with the wrong positional relations among the door, papers, and the black box. Our approach can handle both color and geometric local information better.

 {\noindent\textbf{Ablation Study:}} As Tab.~\ref{tab:rerank_ablation}, we compare our approach with three different modified versions to highlight the benefits of our design. Attention~\cite{vaswani2017attention} composes a sequence of self-attention and cross-attention models to substitute our SCC and CSCC.  {The CoCs concept allows for multi-scale feature processing by relating large-scale environmental representations to small-scale object details, unlike attention mechanisms, which operate at a single scale without multi-scale interactions.} Therefore, our design based on the CoCs concept outperforms attention-based alternatives by at least $11\%$ on ARKitIPR and ScanNetIPR in Recall@1 and is also faster. SCC improves the performance by at least $9\%$ on the two datasets by enhancing the local features with global information. We also observe the correlation matrix is critical in reranking, and improves by at least $65\%$ on two datasets, as discussed in Section \ref{sec:architecture}, which provides the relationship between two frames. These results demonstrate the effect of our innovative components (SCC and CSCC) and the efficacy of generalizing the CoCs concept to RGB-D point cloud for feature processing in RGB-D place recognition reranking.


\section{Conclusion, Limitations, and Future Work}
% \textbf{Conclusion:} 
We explored the RGB-D place recognition with an integrated mechanism for both global retrieval and reranking. By developing a fast and effective reranking model, we close the gap between RGB-D place recognition reranking and learning-based algorithms. We generalized the CoCs concept to noisy colorized point cloud feature processing and demonstrated better performance in place recognition tasks. We handle the scarcity of RGB-D place recognition datasets and propose a data generation pipeline for the community to explore more datasets. We introduce two large-scale RGB-D datasets for training and testing purposes. We push forward the boundary of RGB-D indoor place recognition accuracy by demonstrating our design outperforming other SOTA approaches by at least $36.5$ in Recall@1 in the ScanNet-PR dataset. For limitations, if the overlapping areas do not have many features, our method may not work well. As part of future work, we would like to apply semantic pretraining to the model to improve its understanding of the environment.


